Cosmology from Cosmic Shear with DES Science Verification Data

We present the first constraints on cosmology from the Dark Energy Survey (DES), using weak lensing measurements from the preliminary Science Verification (SV) data. We use 139 square degrees of SV data, which is less than 3\% of the full DES survey area. Using cosmic shear 2-point measurements over three redshift bins we find $\sigma_8 (\Omega_{\rm m}/0.3)^{0.5} = 0.81 \pm 0.06$ (68\% confidence), after marginalising over 7 systematics parameters and 3 other cosmological parameters. We examine the robustness of our results to the choice of data vector and systematics assumed, and find them to be stable. About $20$\% of our error bar comes from marginalising over shear and photometric redshift calibration uncertainties. The current state-of-the-art cosmic shear measurements from CFHTLenS are mildly discrepant with the cosmological constraints from Planck CMB data; our results are consistent with both datasets. Our uncertainties are $\sim$30\% larger than those from CFHTLenS when we carry out a comparable analysis of the two datasets, which we attribute largely to the lower number density of our shear catalogue. We investigate constraints on dark energy and find that, with this small fraction of the full survey, the DES SV constraints make negligible impact on the Planck constraints. The moderate disagreement between the CFHTLenS and Planck values of $\sigma_8 (\Omega_{\rm m}/0.3)^{0.5}$ is present regardless of the value of $w$.

==> Makefile <==
# makefile to make the pdf and bibliography
# 
# This makes the pdf
#     make
# if you add citations, run the following
#     make bib
#     make
#

texfile := main
default: pdf

# run "make bib" when you add new citations
bib: 
	bibtex ${texfile}


# twice to deal with newly added references
pdf:
	pdflatex ${texfile}
	pdflatex ${texfile}

clean:
	rm -f \
	${texfile}.dvi \
	${texfile}.out \
	${texfile}.ps \
	${texfile}.pdf \
	${texfile}.aux \
	${texfile}.bbl \
	${texfile}.blg \
	${texfile}.toc \
	${texfile}.log \
	${texfile}.synctex.gz

diff:
	latexdiff ../paper-prd.31.07.15/main.tex main.tex > diff.tex
	pdflatex diff
	pdflatex diff
	
diffbib:
	bibtex diff
diffclean:
	rm -f \
	diff.dvi \
	diff.out \
	diff.ps \
	diff.pdf \
	diff.aux \
	diff.bbl \
	diff.blg \
	diff.toc \
	diff.log \
	diff.synctex.gz


==> affil.tex <==
$[1]$ Cerro Tololo Inter-American Observatory, National Optical Astronomy Observatory, Casilla 603, La Serena, Chile\\
$[2]$ Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK\\
$[3]$ Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA\\
$[4]$ Department of Physics, ETH Zurich, Wolfgang-Pauli-Strasse 16, CH-8093 Zurich, Switzerland\\
$[5]$ Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA\\
$[6]$ Institute of Cosmology \& Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK\\
$[7]$ Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$[8]$ Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$[9]$ Institut de Ci\`encies de l'Espai, IEEC-CSIC, Campus UAB, Carrer de Can Magrans, s/n,  08193 Bellaterra, Barcelona, Spain\\
$[10]$ Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA\\
$[11]$ Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA\\
$[12]$ Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA\\
$[13]$ Carnegie Observatories, 813 Santa Barbara St., Pasadena, CA 91101, USA\\
$[14]$ Sorbonne Universit\'es, UPMC Univ Paris 06, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$[15]$ CNRS, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$[16]$ Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA\\
$[17]$ Institut de F\'{\i}sica d'Altes Energies, Universitat Aut\`onoma de Barcelona, E-08193 Bellaterra, Barcelona, Spain\\
$[18]$ Jodrell Bank Centre for Astrophysics, School of Physics and Astronomy, University of Manchester, Oxford Road, Manchester, M13 9PL, UK\\
$[19]$ SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA\\
$[20]$ Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$[21]$ Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$[22]$ National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA\\
$[23]$ Department of Astronomy, University of Illinois, 1002 W. Green Street, Urbana, IL 61801, USA\\
$[24]$ Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA\\
$[25]$ George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA\\
$[26]$ Excellence Cluster Universe, Boltzmannstr.\ 2, 85748 Garching, Germany\\
$[27]$ Faculty of Physics, Ludwig-Maximilians University, Scheinerstr. 1, 81679 Munich, Germany\\
$[28]$ Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany\\
$[29]$ Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA\\
$[30]$ Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA\\
$[31]$ Department of Astronomy, University of Michigan, Ann Arbor, MI 48109, USA\\
$[32]$ Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany\\
$[33]$ Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain\\
$[34]$ Department of Physics, The Ohio State University, Columbus, OH 43210, USA\\
$[35]$ Australian Astronomical Observatory, North Ryde, NSW 2113, Australia\\
$[36]$ Argonne National Laboratory, 9700 South Cass Avenue, Lemont, IL 60439, USA\\
$[37]$ Departamento de F\'{\i}sica Matem\'atica,  Instituto de F\'{\i}sica, Universidade de S\~ao Paulo,  CP 66318, CEP 05314-970 S\~ao Paulo, Brazil\\
$[38]$ Department of Astronomy, The Ohio State University, Columbus, OH 43210, USA\\
$[39]$ Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain\\
$[40]$ Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA 94720, USA\\
$[41]$ Department of Physics and Astronomy, Pevensey Building, University of Sussex, Brighton, BN1 9QH, UK\\
$[42]$ Korea Astronomy and Space Science Institute, Yuseong-gu, Daejeon, 305-348, Korea\\
$[43]$ Brookhaven National Laboratory, Bldg 510, Upton, NY 11973, USA\\
$[44]$ Department of Physics, University of Illinois, 1110 W. Green St., Urbana, IL 61801, USA\\
$[45]$ South East Physics Network, (www.sepnet.ac.uk), UK\\
$[46]$ Instituto de F\'{i}sica Te\'{o}rica IFT-UAM/CSIC, Universidad Aut\'{o}noma de Madrid, 28049 Madrid, Spain
$[47]$ Department of Physics and Astronomy, Ohio University, 251B Clippinger Labs, Athens, OH 45701

==> authors.tex <==
% WARNING: Hacking umlaut escape sequence
% WARNING: Blank affiliation for 'M.~T.~Busha'
% WARNING: Blank affiliation for ''
% WARNING: Blank affiliation for ''
% WARNING: Blank affiliation for 'H.~Seo'


\author[The Dark Energy Survey Collaboration]{
\parbox{\textwidth}{
\Large
The Dark Energy Survey Collaboration:
T.~Abbott$^{1}$,
F.~B.~Abdalla$^{2}$,
S.~Allam$^{3}$,
A.~Amara$^{4}$,
J.~Annis$^{3}$,
R.~Armstrong$^{5}$,
D.~Bacon$^{6}$,
M.~Banerji$^{7,8}$,
A.~H.~Bauer$^{9}$,
E.~Baxter$^{10}$,
M.~R.~Becker$^{11,12}$,
A.~Benoit-L{\'e}vy$^{2}$,
R.~A.~Bernstein$^{13}$,
G.~M.~Bernstein$^{10}$,
E.~Bertin$^{14,15}$,
J.~Blazek$^{16}$,
C.~Bonnett$^{17}$,
S.~L.~Bridle$^{18}$,
D.~Brooks$^{2}$,
C.~Bruderer$^{4}$,
E.~Buckley-Geer$^{3}$,
D.~L.~Burke$^{11,19}$,
M.~T.~Busha$^{11,12}$,
D.~Capozzi$^{6}$,
A.~Carnero~Rosell$^{20,21}$,
M.~Carrasco~Kind$^{22,23}$,
J.~Carretero$^{9,17}$,
F.~J.~Castander$^{9}$,
C.~Chang$^{4}$,
J.~Clampitt$^{10}$,
M.~Crocce$^{9}$,
C.~E.~Cunha$^{11}$,
C.~B.~D'Andrea$^{6}$,
L.~N.~da Costa$^{21,20}$,
R.~Das$^{24}$,
D.~L.~DePoy$^{25}$,
S.~Desai$^{26,27}$,
H.~T.~Diehl$^{3}$,
J.~P.~Dietrich$^{28,26}$,
S.~Dodelson$^{3,29}$,
P.~Doel$^{2}$,
A.~Drlica-Wagner$^{3}$,
G.~Efstathiou$^{7,8}$,
T.~F.~Eifler$^{30,10}$,
B.~Erickson$^{24}$,
J.~Estrada$^{3}$,
A.~E.~Evrard$^{24,31}$,
A.~Fausti Neto$^{21}$,
E.~Fernandez$^{17}$,
D.~A.~Finley$^{3}$,
B.~Flaugher$^{3}$,
P.~Fosalba$^{9}$,
O.~Friedrich$^{32,28}$,
J.~Frieman$^{29,3}$,
C.~Gangkofner$^{26,27}$,
J.~Garc\'{i}a-Bellido$^{46}$,
E.~Gaztanaga$^{9}$,
D.~W.~Gerdes$^{24}$,
D.~Gruen$^{32,28}$,
R.~A.~Gruendl$^{22,23}$,
G.~Gutierrez$^{3}$,
W.~Hartley$^{4}$,
M.~Hirsch$^{2}$,
K.~Honscheid$^{16,34}$,
E.~M.~Huff$^{16,34}$,
B.~Jain$^{10}$,
D.~J.~James$^{1}$,
M.~Jarvis$^{10}$,
T.~Kacprzak$^{4}$,
S.~Kent$^{3}$,
D.~Kirk$^{2}$,
E.~Krause$^{11}$,
A.~Kravtsov$^{29}$,
K.~Kuehn$^{35}$,
N.~Kuropatkin$^{3}$,
J.~Kwan$^{36}$,
O.~Lahav$^{2}$,
B.~Leistedt$^{2}$,
T.~S.~Li$^{25}$,
M.~Lima$^{21,37}$,
H.~Lin$^{3}$,
N.~MacCrann$^{18}$ \thanks{Corresponding author:\newline \texttt{niall.maccrann@postgrad.manchester.ac.uk}},
M.~March$^{10}$,
J.~L.~Marshall$^{25}$,
P.~Martini$^{16,38}$,
R.~G.~McMahon$^{7,8}$,
P.~Melchior$^{34,16}$,
C.~J.~Miller$^{31,24}$,
R.~Miquel$^{39,17}$,
J.~J.~Mohr$^{32,27,26}$,
E.~Neilsen$^{3}$,
R.~C.~Nichol$^{6}$,
A.~Nicola$^{4}$,
B.~Nord$^{3}$,
R.~Ogando$^{21,20}$,
A.~Palmese$^{2}$,
H.V.~Peiris$^{2}$,
A.~A.~Plazas$^{30}$,
A.~Refregier$^{4}$,
N.~Roe$^{40}$,
A.~K.~Romer$^{41}$,
A.~Roodman$^{19,11}$,
B.~Rowe$^{2}$,
E.~S.~Rykoff$^{11,19}$,
C.~Sabiu$^{42}$,
I.~Sadeh$^{2}$,
M.~Sako$^{10}$,
S.~Samuroff$^{18}$,
C.~S{\'a}nchez$^{17}$,
E.~Sanchez$^{33}$,
H.~Seo$^{16,47}$,
I.~Sevilla-Noarbe$^{33,23}$,
E.~Sheldon$^{43}$,
R.~C.~Smith$^{1}$,
M.~Soares-Santos$^{3}$,
F.~Sobreira$^{3,21}$,
E.~Suchyta$^{34,16}$,
M.~E.~C.~Swanson$^{22}$,
G.~Tarle$^{24}$,
J.~Thaler$^{44}$,
D.~Thomas$^{6,45}$,
M.~A.~Troxel$^{18}$,
V.~Vikram$^{36}$,
A.~R.~Walker$^{1}$,
R.~H.~Wechsler$^{19,11,12}$,
J.~Weller$^{32,26,28}$,
Y.~Zhang$^{24}$,
J.~Zuntz$^{18}$\thanks{Corresponding author:\newline \texttt{joseph.zuntz@manchester.ac.uk}}
\begin{center} \emph{(Affiliations may be found in Appendix \ref{sec:affiliations})} \end{center}
}
}
